Utilizing Strategic Pre-training to Reduce Overfitting: Baguan -- A Pre-trained Weather Forecasting Model

Weather forecasting has long posed a significant challenge for humanity. While recent AI-based models have surpassed traditional numerical weather prediction (NWP) methods in global forecasting tasks, overfitting remains a critical issue due to the limited availability of real-world weather data spanning only a few decades. Unlike fields like computer vision or natural language processing, where data abundance can mitigate overfitting, weather forecasting demands innovative strategies to address this challenge with existing data. In this paper, we explore pre-training methods for weather forecasting, finding that selecting an appropriately challenging pre-training task introduces locality bias, effectively mitigating overfitting and enhancing performance. We introduce Baguan, a novel data-driven model for medium-range weather forecasting, built on a Siamese Autoencoder pre-trained in a self-supervised manner and fine-tuned for different lead times. Experimental results show that Baguan outperforms traditional methods, delivering more accurate forecasts. Additionally, the pre-trained Baguan demonstrates robust overfitting control and excels in downstream tasks, such as subseasonal-to-seasonal (S2S) modeling and regional forecasting, after fine-tuning.

==> sections/3.2-therotical_analysis.tex <==
\section{Pre-training as Regularization}

In this section, we focus on linear regression to understand how pre-training acts as a regularization mechanism that mitigates the overfitting problem. We demonstrate that pre-training effects analogous to pruning the subspace spanned by eigenvectors with small eigenvalues, hence regularizing the final solution to rely primarily on the leading eigenvectors of the covariance matrix. This regularization enhances generalization when the target solution resides within the subspace of leading eigenvectors.

We begin with the standard setup of linear regression. For a set of training examples $(x_i, y_i)$ where $x_i \in \mathbb{R}^d$ and $y_i \in \mathbb{R}$, and a covariance matrix $\Sigma = \mathbb{E}[x_ix_i^{\top}]$, we consider an optimal weight vector $w_*$ in the subspace spanned by the top $K$ eigenvectors of $\Sigma$. Through analysis, we establish that pre-training, particularly using a denoising model, can enhance generalization performance.

Key findings:

\begin{enumerate}
    \item Without pre-training, the error bound for the estimated weights, considering the top $K$ eigenvectors, is given by:
    \begin{equation}
        |w_1 - w_*| \leq \frac{\lambda}{R^2/2\sqrt{K} + \lambda} |w_*| + \frac{R}{n} + \sqrt{\frac{\sigma^2Rd^{1/2}}{n}\log\frac{1}{\delta}}. 
    \end{equation}
    \item By employing a pre-training method (denoising),  with high probability the error bound becomes:
    \begin{equation}
        |w_2 - w_*| \leq O\sqrt{\frac{1}{n}}, 
    \end{equation}
\end{enumerate}
indicating significant improvement in generalization error. Detailed derivations and proofs supporting these results are provided in Appendix~\ref{appendix_provement}.

==> tables/0_highlight.tex <==
\begin{table}[t]
\caption{Highlights}
\label{sample-table}
\begin{center}
% \begin{tiny}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \resizebox{1\textwidth}{!}
{
\begin{tabular}{|cc|cccccc|}
\hline
\textbf{Model} & \textbf{Time} & \textbf{S2S} & \textbf{Regional forecast} \\
\hline
Baguan & 1h & $\checkmark$ & $\checkmark$  \\
Pangu & 1h & $\times$ & $\times$  \\
Fuxi \& Fuxi2.0 & 1h & $\checkmark$ \\
Fengwu & 6h & $\times$\\
GraphCast & 6h & $\times$ \\



\hline
% \textbf{Total} & & & & & & \textbf{1,219.91} & \textbf{11,023,730} \\
% \hline
\end{tabular}
}
% \end{tiny}
\end{center}
\end{table}



==> tables/1_benchmark.tex <==
\begin{table}[t]
\caption{Benchmark}
\label{sample-table}
\begin{center}
\begin{tiny}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{lllllllllllll}
\multirow{2}{*}{t} & \multirow{2}{*}{variables} & \multicolumn{3}{l}{Ours}     & \multicolumn{2}{l}{ClimaX} & FCN    & Pangu  & GC     & HRES   & \multicolumn{2}{l}{IFS} \\

                           &                            & 5.6 & 1.4  & 0.25 & 5.6       & 1.4      & 0.25   & 0.25   & 0.25   & 0.1    & 5.6        & 1.4deg     \\
\hline
6                          & Z500                       & 44.72    & 38.642  &         & 62.73        & 49.67       & 37.52  & 15.4   & 16.46  & 24.66  & 26.93      & 26.96      \\
                           & T2m                        & 0.8478   & 0.6916  &         & 0.95         & 1.11        & 0.72   & 0.59   & 0.50   & 0.35   & 0.97       & 0.97       \\
                           & T850                       & 0.7857   & 0.5728  &         & 0.88         & 0.84        & 0.52   & 0.42   & 0.28   & 0.33   & 0.69       & 0.69       \\
                           & U10                        & 0.8862   & 0.6284  &         & 1.08         & 1.04        & 0.55   & 0.46   & 0.37   & 0.58   & 0.80       & 0.80       \\
\hline
24                         & Z500                       & 76.48    & 60.059  &         & 96.19        & 72.76       & 81.31  & 42.23  & 38.77  & 45.90  & 51.01      & 50.96      \\
                           & T2m                        & 1.079    & 1.031   &         & 1.10         & 1.19        & 0.95   & 0.72   & 0.62   & 0.66   & 1.02       & 1.02       \\
                           & T850                       & 1.013    & 0.8759  &         & 1.11         & 1.02        & 0.81   & 0.72   & 0.58   & 0.70   & 0.87       & 0.87       \\
                           & U10                        & 1.229    & 1.04    &         & 1.41         & 1.31        & 0.99   & 0.9    & 0.80   & 1.15   & 1.11       & 1.11       \\
\hline
72                         & Z500                       & 207.8    & 168.429 &         & 244.08       & 201.00      & 251.96 & 133.12 & 125.78 & 146.37 & 152.15     & 152.20     \\
                           & T2m                        & 1.458    & 1.2834  &         & 1.43         & 1.47        & 1.38   & 1.05   & 0.94   & 1.06   & 1.30       & 1.30       \\
                           & T850                       & 1.434    & 1.2514  &         & 1.59         & 1.46        & 1.55   & 1.13   & 1.02   & 1.27   & 1.34       & 1.34       \\
                           & U10                        & 1.971    & 1.7216  &         & 2.18         & 2.02        & 2.24   & 1.6    & 1.47   & 1.98   & 1.92       & 1.92       \\
\hline
120                        & Z500                       & 381.9    & 331.561 &         & 440.40       & 392.00      & 483.44 & 295.63 & 271.65 & 316.79 & 331.45     & 331.38     \\
                           & T2m                        & 1.917    & 1.6487  &         & 1.83         & 1.83        & 1.99   & 1.53   & 1.36   & 1.52   & 1.72       & 1.71       \\
                           & T850                       & 2.034    & 1.8332  &         & 2.23         & 2.08        & 2.47   & 1.78   & 1.63   & 1.96   & 2.01       & 2.01       \\
                           & U10                        & 2.714    & 2.4910  &         & 2.94         & 2.79        & 3.41   & 2.52   & 2.36   & 2.95   & 2.89       & 2.89       \\
\hline
168                        & Z500                       & 545      &         &         & 599.43       & 566.00      & 680.00 & 504.90 & 466.53 & 535.93 & 549.01     & 548.96     \\
                           & T2m                        & 2.274    &         &         & 2.18         & 2.17        & 2.54   & 2.06   & 1.88   & 2.06   & 2.24       & 2.23       \\
                           & T850                       & 2.603    &         &         & 2.77         & 2.66        & 3.30   & 2.60   & 2.41   & 2.78   & 2.82       & 2.82       \\
                           & U10                        & 3.265    &         &         & 3.43         & 3.35        & 4.18   & 3.46   & 3.25   & 3.87   & 3.81       & 3.81      
% \hline
\end{tabular}
\end{tiny}
\end{center}
\end{table}



==> tables/6_gflops.tex <==
% \begin{table}[h]
% \centering

% \end{table}

\begin{table}[t]
\caption{Efficiency study}
\label{sample-table}
\begin{center}
% \begin{tiny}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\resizebox{1\textwidth}{!}{

\begin{tabular}{|l|c|l|c|c|}
\hline
\textbf{Model} & \textbf{Number of predictands} & \textbf{Resolution (all have 0.25° spatial resolution)} & \textbf{Parameters} & \textbf{Computational complexity*} \\ \hline
Pangu-Weather & 69 & Vertical: 13 pressure level and surface & 740 million & 4950 Gflops \\ 
 & & Frequency: 1h, 3h, 6h, 24h & & \\ \hline
GraphCast & 227 & Vertical: 37 pressure level and surface & 55 million & 13564 Gflops \\ 
 & & Frequency: 6h & & \\ \hline
FengWu & 189 & Vertical: 37 pressure level and surface & 751 million & 8000 Gflops \\ 
 & & Frequency: 6h & & \\ \hline
FuXi & 70 & Vertical: 13 pressure level and surface & 1556 million & 19892 Gflops \\ 
 & & Frequency: 6h & & \\ \hline
Baguan & 13 & & 2900 million & xxx Gflops \\ 
\hline
% \textbf{Total} & & & & & & \textbf{1,219.91} & \textbf{11,023,730} \\
% \hline
\end{tabular}
}
% \end{tiny}
\end{center}
\end{table}



==> tables/7_pretraing_exp.tex <==
\begin{table}[h]
\caption{RMSE of Various Pre-training Methods on $5.625^\circ$ data. Key variables analyzed include U10, T2M, Y850 and Z500. Lower RMSE is better.}
\label{tab:pretrain_exp_5}
\begin{center}
\begin{tabular}{lllllll}

\toprule
& Lead Time & U10  & T2M & T850 & Z500 \\
& (hr.) & ($m/s$) & ($K$) & ($K$) & ($m^2/s^2$) \\
\midrule
\multirow{2}{*}{ClimaX} 
& 6 & 1.08 & 0.95 & 0.88 & 62.73\\
& 24 & 1.41 & 1.10 & 1.11 & 96.19\\
% & 72 & 2.18 & 1.43 & 1.59 & 244.08\\
\midrule
\multirow{2}{*}{MAE} 
& 6 & 0 & 0 & 0 & 0\\
& 24 & 0 & 0 & 0 & 0\\
% & 72 & 0 & 0 & 0 & 0\\
\midrule
\multirow{2}{*}{\NAME} 
& 6 & 0.88 & 0.84 & 0.78 & 44.72\\
& 24 & 1.22 & 1.07 & 1.01 & 76.48\\
% & 72 & 1.97 & 1.45 & 1.43 & 207.80\\
\bottomrule
 



% \\ \hline \\
% Dendrite         &Input terminal \\
% Axon             &Output terminal \\
% Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\begin{table}[h]
\caption{RMSE of Various Pre-training Methods on $1.40625^\circ$ data. Key variables analyzed include U10, T2M, Y850 and Z500. Lower RMSE is better.}
\label{tab:pretrain_exp_1}
\begin{center}
\begin{tabular}{lllllll}

\toprule
& Lead Time & U10  & T2M & T850 & Z500 \\
& (hr.) & ($m/s$) & ($K$) & ($K$) & ($m^2/s^2$) \\
\midrule
\multirow{2}{*}{ClimaX} 
& 6 & 1.04 & 1.11 & 0.84 & 49.67 \\
& 24 & 1.31 & 1.19 & 1.02 & 72.76 \\
% & 72 & 2.02 & 1.47 & 1.46 & 201.00 \\
\midrule
\multirow{2}{*}{MAE} 
& 6 & 0 & 0 & 0 & 0\\
& 24 & 0 & 0 & 0 & 0\\
% & 72 & 0 & 0 & 0 & 0\\
\midrule
\multirow{2}{*}{\NAME} 
& 6 & 0.62 & 0.69 & 0.57 & 38.64 \\
& 24 & 1.04 & 1.03 & 0.87 & 60.06 \\
% & 72 & 1.72 & 1.28 & 1.25 & 168.43 \\
\bottomrule
 



% \\ \hline \\
% Dendrite         &Input terminal \\
% Axon             &Output terminal \\
% Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}
